Understanding Edge-of-Stability Training Dynamics with a Minimalist Example

Recently, researchers observed that gradient descent for deep neural networks operates in an ``edge-of-stability'' (EoS) regime: the sharpness (maximum eigenvalue of the Hessian) is often larger than stability threshold $2/\eta$ (where $\eta$ is the step size). Despite this, the loss oscillates and converges in the long run, and the sharpness at the end is just slightly below $2/\eta$. While many other well-understood nonconvex objectives such as matrix factorization or two-layer networks can also converge despite large sharpness, there is often a larger gap between sharpness of the endpoint and $2/\eta$. In this paper, we study EoS phenomenon by constructing a simple function that has the same behavior. We give rigorous analysis for its training dynamics in a large local region and explain why the final converging point has sharpness close to $2/\eta$. Globally we observe that the training dynamics for our example has an interesting bifurcating behavior, which was also observed in the training of neural nets.

==> 4Num_Example/12step_dynamics.tex <==
\subsection{One and Two Step Dynamics of $c$ and $d$}
Now with the notations defined we can proceed to analyze the dynamics of $(c_{(t)},d_{(t)}).$
For simplicity of notations, when analyzing the one-step and two-step dynamics of $(c_{(t)}, c_{(t)})$, we use $c, c', c''$ to denote $c_{(t)}, c_{(t+1)}, c_{(t+2)}$ and $d, d', d''$ to denote $d_{(t)}, d_{(t+1)}, d_{(t+2)}$.

We consider the situation with small $\eta$. Let $|c|=\Theta(\eta^\alpha)$ and $d=\Theta(\eta^\beta)$. We first consider the regime in which $\alpha\in (0,2]$ and $\beta\in(0,\infty)$, which corresponds to the region with smaller than constant distance from the sharpest stable minima, and $|c|$ is not too small. Let 
\begin{equation}
    \delta\triangleq \sqrt{4\eta^2 (1+c)^2+\rbr{d\eta^{\frac12}+(1 - 4\eta^2)^{\frac14}}^4}
    \label{eqn:4num-delta-def}
\end{equation}
Plugging \cref{eqn:4num-delta-def} into \cref{eqn:4num-cd-dynamics} we have \begin{equation}
\begin{split}
    c'=&\ c-2 c \delta -3 c^2 \delta -c^3 \delta +4 c^2 \eta ^2+16 c^3 \eta ^2+25
   c^4 \eta ^2+19 c^5 \eta ^2+7 c^6 \eta ^2+c^7 \eta ^2\\
   =&\ c-2 c \delta -3 c^2 \delta -c^3 \delta +4 c^2 \eta ^2 + O\rbr{\eta^{2+3\alpha}}.
   % +O\rbr{\eta^{2+2\alpha}}.
   \label{eqn:4num-cprime-delta-1}
\end{split}
\end{equation}
By Taylor expansion on $\delta$  we have \begin{equation}
    \delta = 1+ 2d\eta^{\frac12} + d^2\eta + 4c\eta^2 + 2c^2\eta^2 - 6d\eta^{\frac52} + O\rbr{\eta^{\min\cbr{\frac52+\alpha, 3+\beta, \frac92}}}.
    \label{eqn:4num-delta-taylor}
\end{equation}
Plugging \cref{eqn:4num-delta-taylor} into \cref{eqn:4num-cprime-delta-1}, we have \begin{equation}
\begin{split}
    c' =&  -c - 4cd\eta^{\frac12}-2cd^2\eta+12cd\eta^{\frac52}-3c^2 - 6c^2d\eta^{\frac12} - 3cd^2\eta\\
    &\ - c^3 - 2c^3d\eta^{\frac12}-c^3d^2\eta + 4c^2\eta^2 + O\rbr{\eta^{\min\cbr{2+3\alpha, \frac52+2\alpha, \frac92+\alpha, 3+\alpha+\beta}}}\\
    =& -c-4cd\eta^{\frac12} -3c^2-c^3 + 4c^2\eta^2 + O\rbr{\eta^{\min\cbr{1+\alpha+\beta, \frac12+\frac32\alpha+\beta,\frac12+3\alpha}}}.
    \label{eqn:4num-cprime-delta-1}
\end{split}
\end{equation}
The last step holds since we only consider $\alpha\leq 2$, thus $\frac92+\alpha \geq \frac52+2\alpha\geq \frac12+3\alpha$ and $\frac12+\frac32\alpha+\beta < 3+\alpha+\beta$.

Similarly, by a Taylor expansion on $d'$, we have \begin{equation}
    d'= d - 2c^2\eta^{\frac32} + O\rbr{\eta^{\min\cbr{3\alpha + \frac32, 2\alpha + 2, \frac{13}{2}}}}.
\end{equation}
For the two step dynamics, we have
\begin{equation}
\begin{split}
    c''=& -c'-4c'd'\eta^{\frac12} -3c'^2-c'^3 + 4c'^2\eta^2 + O\rbr{\eta^{\min\cbr{1+\alpha+\beta,\frac12+\frac32\alpha+\beta,\frac12+3\alpha}}}.\\
    =&\ \srbr{c + 3c^2 + c^3 + 4cd\eta^{\frac12} - 4c^2\eta^2} + 4\srbr{cd\eta^{\frac12}}\\
    &\ - 3\srbr{c^2+6c^3} - \srbr{-c^3} + 4\srbr{c^2\eta^2}+ O\rbr{\eta^{\min\cbr{1+\alpha+\beta,\frac12+\frac32\alpha+\beta,\frac12+3\alpha}}}\\
    =&\ c + 8cd\eta^{\frac12} - 16c^3 + O\rbr{\eta^{\min\cbr{1+\alpha+\beta,\frac12+\frac32\alpha+\beta,\frac12+3\alpha}}}.
    \label{eqn:4num-2step-c-dynamics}
\end{split}
\end{equation}
and
\begin{equation}
\begin{split}
    d'' =&\ d'-2c'^2\eta^{\frac32} + O\rbr{\eta^{\min\cbr{3\alpha + \frac32, 2\alpha + 2, \frac{13}{2}}}}\\
    =&\ d-2c^2\eta^{\frac32} - 2\srbr{c^2\eta^{\frac32}}+ O\rbr{\eta^{\min\cbr{3\alpha + \frac32, 2\alpha + 2, \frac{13}{2}}}}\\
    =&\ d-4c^2\eta^{\frac32}+ O\rbr{\eta^{\min\cbr{3\alpha + \frac32, 2\alpha + 2, \frac{13}{2}}}}.
    \label{eqn:4num-2step-d-dynamics}
\end{split}
\end{equation}

==> 4Num_Example/ODE_approx.tex <==
\subsection{Exponential Function, Parabola, and Ellipse}
Before we proceed to the rigorous derivation with discrete updates, let us first build up some intuitions on the 2-step dynamics using an ODE approximation, namely
\begin{equation}
    \frac{\text{d} c}{\text{d} d} = \frac{4c^3 - 2cd\eta^{\frac12}}{c^2\eta^{\frac32}}.
    \label{eqn:4num-ode-approx}
\end{equation}
Depending on the relation between $c$ and $d$, the ODE presents three different behaviors
\begin{enumerate}
    \item When $c=o\srbr{d^{\frac12}\eta^{\frac14}}$, $2cd\eta^{\frac12}$ dominates $4c^3$. The approximate ODE gives the solution family \begin{equation}
        c=\pm \sqrt{\frac{2}{\eta}}\sqrt{\gamma - d^2}
    \end{equation}
    for some constant $\gamma$. These are ellipses with eccentricity $\sqrt{1-2/\eta}$ centered at the sharpest stable minima. As $d$ decreases, $|c|$ increases quadratically with the movement of $d$.
    
    \item When $c=\omega\srbr{d^{\frac12}\eta^{\frac14}}$, $4c^3$ dominates $2cd\eta^{\frac12}$, the ODE reduces to $c'=4c\eta^{-\frac32}$. This gives the solution family of exponential functions
    \begin{equation}
        c=\gamma\exp\rbr{4d\eta^{-\frac32}}
    \end{equation} 
    for some constant $\gamma$. As $d$ decreases, $|c|$ decreases exponentially with the movement of $d$.

    \item When $c=\Theta(d^{\frac12}\eta^{\frac14})$, the ODE gives the solution family
    \begin{equation}
        c = \pm\sqrt{\frac12 d\eta^{\frac12} + \frac{1}{16}\eta^2 + \gamma\exp\rbr{8d \eta^{-\frac32}}}
    \end{equation}
    for some constant $\gamma$. When $\gamma=0$, this gives a parabola parameterized by $c^2=\frac12 d\eta^{\frac12} +\frac{1}{16}\eta^2.$
\end{enumerate}


==> 4Num_Example/corollaries/cor_adaptive.tex <==
We first restate \cref{cor:MT-4Num-adaptive} here


==> 4Num_Example/corollaries/cor_xy_regime.tex <==
We first restate \cref{cor:MT-4Num-convergence-xysharp} here. 

\begin{corollary}[Region of EoS Initializations under $x,y$-Parameterization]
There exists some absolute constant $K$ such that for all step size $\eta < \frac{1}{8000000}K^{-2}$, for all initialization $(x_0, y_0)$ satisfying $x_0\in (\breve x + 3\eta^{\frac54}, \breve x + \frac14 K^{-2}\eta^{-\frac12})$ and $|x_0y_0-1|<K^{-1}$ where $(\breve x, \breve y)$ is the $\eta$-EoS minima defined in \cref{def:MT-EoS-Min}, following gradient descent with constant step size $\eta$ characterized by \cref{eqn:MT-4Num-update}, it will converge to a global minimum with sharpness $\lambda \in (\tfrac{2}{\eta} - \tfrac{20}{3}\eta, \tfrac{2}{\eta})$
\label{cor:APDX-4Num-convergence-xysharp}
\end{corollary}

\begin{proof}
Following the convergence proof for \cref{thm:APDX-4Num-convergence-ab}, to prove this corollary we only need to show that all initializations $x_0, y_0$ satisfies the initialization condition of \cref{thm:APDX-4Num-convergence-ab} after re-parameterized to $(a, b)$, and the sharpness $\lambda$ of the minima will satisfy $\lambda \in (XX, XX)$.

We first check TBC

Now we show that for global minima with satisfies $a_k \in [-\frac53, -\frac{9}{50}]$ and $b_k = 0$, the sharpness $\lambda$ satisfies xxx.

Recall from \cref{eqn:MT-xy-sharpness} that the sharpness of $(x,y)$ near the global minima is given by
\begin{equation}
    \lambda = \tfrac12\rbr{\rbr{x^2+y^2}\rbr{3\gamma^2-1} + \sqrt{(x^2 + y^2)^2 (1 - 3 \gamma^2)^2 + 4 \gamma^2(3 - 10 \gamma^2+ 7 \gamma^4)}}
\label{eqn:APDX-xy-sharpness-restate}
\end{equation}
where $\gamma \triangleq xy$, when $(x,y)$ is a global minima, $\gamma=1$, and \cref{eqn:APDX-xy-sharpness-restate} reduces to 
\begin{equation}
\begin{split}
    \lambda &= \tfrac12\rbr{\rbr{x^2+y^2}\rbr{3-1} + \sqrt{(x^2 + y^2)^2 (1 - 3)^2}}\\
    &= \tfrac12(2(x^2+y^2) + 2(x^2+y^2))\\
    &= 2(x^2+y^2)\\
    &= 2\sqrt{(x^2+x^{-2})^2}\\
    &= 2\sqrt{4+ (x^2 - x^{-2})^2}\\
    &= 2\sqrt{4 + (\sqrt{x^2 - y^2})^4}\\
    &= 2\sqrt{4 + c^4}.
\end{split}
\end{equation}
Since $c = (\kappa^{-4} - 4)^{\frac14} + a$, where $a \in [-\frac53\kappa^3, -\frac{9}{50}\kappa^3]$, we have $c < (\kappa^{-4} - 4)^{\frac14}$ and hence $\lambda = 2\sqrt{4+c^4} < 2\sqrt{4 + \kappa^{-4} - 4} = 2\kappa^{-2} = \frac{2}{\eta}$.

Now we prove the lower bound for $\lambda$. Follow from $c > (\kappa^{-4} - 4)^{\frac14} - \frac53\kappa^3$, we have
\begin{equation}
\begin{aligned}
    c^4 >&\ \rbr{(\kappa^{-4} - 4)^{\frac14} - \tfrac53\kappa^3}^4\\
    =&\ \rbr{(\kappa^{-4} - 4)^{-\frac14}(\kappa^{-4} - 4)^{\frac14} - \tfrac53\kappa^3(\kappa^{-4} - 4)^{-\frac14}}^4 (\kappa^{-4} - 4)\\
    =&\ \rbr{1 - \tfrac53\kappa^3(\kappa^{-4} - 4)^{-\frac14}}^4 (\kappa^{-4} - 4)\\
    \geq&\ \rbr{1 - \tfrac{20}{3}\kappa^3(\kappa^{-4} - 4)^{-\frac14}}(\kappa^{-4} - 4) & (\text{Bernoulli inequality})\\
    =&\ \kappa^{-4} - 4 - \tfrac{20}{3}\kappa^3(\kappa^{-4} - 4)^{\frac34}\\
    \geq&\ \kappa^{-4} - 4 - \tfrac{20}{3}\kappa^3(\kappa^{-4})^{\frac34}\\
    =&\ \kappa^{-4} - 4 - \tfrac{20}{3}.
\end{aligned}
\end{equation}
Thus
\begin{equation}
\begin{aligned}
    \lambda &=\ 2\sqrt{4+c^4}\\
    &\geq\ 2\sqrt{4 + \kappa^{-4} - 4 - \tfrac{20}{3}}\\
    &= 2\sqrt{\kappa^{-4} - \tfrac{20}{3}}\\
    &= 2\sqrt{1-\tfrac{20}{3}\kappa^4}\kappa^{-2}\\
    &\geq 2 (1-\tfrac{20}{3}\kappa^4) \kappa^{-2}\\
    &= 2\kappa^{-2} - \tfrac{20}{3}\kappa^2\\
    &= \tfrac{2}{\eta} - \tfrac{20}{3}\eta.
\end{aligned}
\end{equation}
Hence in conclusion, the converging minima has sharpness $\lambda \in (\frac{2}{\eta} - \frac{20}{3}\eta, \frac{2}{\eta})$, which completes the proof for the corollary.
\end{proof}


==> 4Num_Example/main_thm/diagram_placeholder.tex <==
\input{4Num_Example/diagrams/converging_diagram.tex}

==> 4Num_Example/parabola_convergence.tex <==

\subsection{Convergence to Parabola}
Now we show that for initializations with $\alpha\in (0,2]$ and $\beta<\tau$ where $\tau=\frac32-3\kappa$ for some small constant $\kappa$, the trajectory converges to near the parabola $c^2=\frac12 d\eta^{\frac12}+\frac{1}{16}\eta^2$ very fast. Formally,
\begin{theorem}
    For initialization $(c,d)\in\R\times\R^+$ such that $c=\Omega\srbr{\eta^2}$ and $\log_\eta d < \frac32-3\kappa$ for some small constant $\kappa$. $(c,d)$ will enter the regime of $c=\Theta\srbr{d^{\frac12}\eta^{\frac14}}$ within $O(d^{-1}\eta^{\kappa-\frac12})$ steps.
\end{theorem}
\begin{proof}
We consider two cases, $\alpha \in (0, \frac14+\frac12\beta)$ and 
% \textbf{Phase I (2$\to$3)}
% We consider the case with $\beta \in (0,\frac32)$ and $\alpha < \frac14+\frac12\beta$. 

\begin{lemma}[Phase I (2$\to$3)]
    WLOG we only consider the case with positive $c$ in this scenario since $c''$ and $d''$ are symmetric wrt $c$.
    For any constant $\kappa < 1$, for any initialization satisfying $\beta<\frac32 - 3\kappa$ and $\alpha \in (0, \frac14+\frac12\beta)$, following the two step dynamics in \cref{eqn:4num-2step-c-dynamics} and \cref{eqn:4num-2step-d-dynamics}, $c$ will enter $O\srbr{\eta^{\frac14+\frac12\beta}}$ while $d$ remains $\Theta\srbr{\eta^\beta}$.
    \label{lemma:4num-exp-converge}
\end{lemma}

\begin{proof}
When $\alpha \in (0, \frac14+\frac12\beta)$, $c^3$ will dominate $cd\eta^{\frac12}$, thus
\begin{equation}
c''=c-16c^3+O(\eta^{\min\cbr{\frac12+\alpha+\beta, \frac12+3\alpha}}).
\end{equation}
We consider the convergence of $c$ in $\lceil\srbr{\alpha-\frac14-\frac12\beta}/\kappa\rceil$ steps. In the $i$-th phase, we have $c$ decreasing from $\Theta\srbr{\eta^{\alpha+(i-1)\kappa}}$ to $\Theta\srbr{\eta^{\min\cbr{\alpha+i\kappa, \frac14+\frac12\beta}}}$
% \textcolor{red}{should be $\max$ and `+'?}
.
In the $i$-th phase, $c = \Omega\srbr{\eta^{\alpha+i\kappa}},$ thus $c-c''=\Omega\srbr{\eta^{3\alpha+3i\kappa}}.$ Since the total distance for $c$ to travel in this phase is  $O\srbr{\eta^{\alpha+(i-1)\kappa}}$, the number of 2-step updates in the $i$-th phase is
$O\srbr{\eta^{\alpha+(i-1)\kappa}}/\Omega\srbr{\eta^{3\alpha+3i\kappa}} = O\srbr{\eta^{-2(\alpha+i\kappa)-\kappa}}$.
Now we consider the movement of $d$ in phase $i$. Recall that 
\begin{equation}
d''=d-4c^2\eta^{\frac32}+ O\srbr{\eta^{\min\cbr{3\alpha + \frac32, 2\alpha + 2, \frac{13}{2}}}}.
\end{equation}
Since $c=O\srbr{\eta^{\alpha+(i-1)\kappa}}$, the single step movement for $d$ in each 2-step update is bounded by $4c^2\eta^{\frac32} = O(\eta^{2\alpha+2(i-1)\kappa+\frac32})$. By the upper bound on the number of steps from above, the total movement of $d$ in phase $i$ is $O(\eta^{2\alpha+2(i-1)\kappa+\frac32})O\srbr{\eta^{-2(\alpha+i\kappa)-\kappa}} = O\srbr{\eta^{\frac32-3\kappa}}$. Note that this is independent from $i$. Therefore by considering all phases together, with $\kappa$ being some small constant, the total movement of $d$ until $c$ decreases to $\Theta\srbr{\eta^{\frac14+\frac12\beta}}$ is of $O\srbr{\eta^{\frac32-3\kappa}}$. Hence if $\beta < \frac32+3\kappa$, $d$ is still $\Theta\srbr{\eta^\beta}$ after the movement.
\end{proof}

Here note that the $c^2$ update is $c ''^2=c^2(1-16c^2)$, which is very similar to the logistical map.

\begin{lemma}[Phase I (1$\to$3)]
For some constant $\kappa < 1$, for initialization satisfying $\beta < 3/2+\kappa$ and $\alpha\in (\frac14+\frac12\beta, 2]$, $c$ will enter $\Omega(\eta^{\frac14+\frac12\beta})$ while $d$ remains $\Theta(\eta^\beta)$.
\end{lemma}
\begin{proof}
When $\alpha\in(\frac14+\frac12\beta, 2]$, $cd\eta^{\frac12}$ will dominate $c^3$. Therefore,
\begin{equation}
c''=c+8cd\eta^{\frac{1}{2}}+O(\eta^{\min\cbr{3\alpha, 1+\alpha+\beta}}).
\end{equation}

We consider the convergence of $c$ in $\lceil\srbr{-\alpha+\frac14+\frac12\beta}/\kappa\rceil$ steps. In the $i$-th step, we have $c$ increase from $\Theta(\eta^{\alpha-(i-1)\kappa}) $ to $\Theta(\eta^{\max\cbr{\alpha-i\kappa, \frac14+\frac12\beta}})$. The movement of $c$ (multiplicative) is $\eta^{-\kappa}$. By induction, we assume $d=\Theta(\eta^\beta)$ at step $i$ and prove it at step $i+1$. Thus this phase takes convergence time $t=\Theta(\eta^{-\kappa-\beta-\frac12})$.

In the $i$-th phase, $c = O\srbr{\eta^{\alpha-(i-1)\kappa}},$ thus $c^2\eta^{3/2}=O\srbr{\eta^{2\alpha-2(i-1)\kappa+3/2}}$. Recall that
\begin{equation}
d''=d-4c^2\eta^{\frac32}+ O\srbr{\eta^{\min\cbr{3\alpha + \frac32, 2\alpha + 2, \frac{13}{2}}}}.
\end{equation}

The total movement of $d$ is $O(\eta^{2\alpha-2(i-1)\kappa+3/2-\kappa-\beta-1/2})=O(\eta^{2\alpha-(2i-1)\kappa-\beta+1})$. By the definition of $i$, we know $2\alpha-(2i-1)\kappa > \beta+1/2-\kappa$. Thus $2\alpha-(2i-1)\kappa-\beta+1>\frac{3}{2}+\kappa>\beta$, and the movement dominated by $d=\Theta(\eta^{\beta})$. Therefore if $\beta < \frac{3}{2}-\kappa$, d is still $\Theta(\eta^\beta)$ after this movement ($i$+1 step).
\end{proof}

Proving the two lemmas above completes the proof of the theorem.
\end{proof}


\textbf{Phase II}

Define \begin{equation}
    \Delta\triangleq c^2-\frac12d\eta^{\frac12}+\frac{1}{16}\eta^2.
\end{equation}
Let $\Delta''$ be defined accordingly with $c''$ and $d''$, then \begin{equation}
\begin{split}
    \Delta'' =&\ c''^2-\frac12d''\eta^{\frac12} + \frac{1}{16}\eta^2\\
    =&\ c^2-32 c^4+256 c^6+16 c^2 d \sqrt{\eta }-256 c^4 d \sqrt{\eta }+64 c^2d^2 \eta \\
    &+ O\rbr{\eta^{\min\cbr{1+2\alpha+\beta,\frac12+\frac52\alpha+\beta,\frac12+4\alpha}}}\\
    &-\frac12d\eta^{\frac12} + 2c^2\eta^2 + O\rbr{\eta^{\min\cbr{3\alpha + \frac32, 2\alpha + 2, \frac{13}{2}}}} + \frac{1}{16}\eta^2\\
    =&\ \Delta - 32c^4 + O\rbr{\eta^{\min\cbr{\frac12+\frac52\alpha+\beta,\frac12+4\alpha, 2\alpha + 2, 5\alpha}}}.
\end{split}
\end{equation}
The last step holds since $\alpha < 1$, so $\frac12+\frac52\alpha+\beta < 1+2\alpha+\beta$ and $4\alpha + \frac12 < 3\alpha + \frac32$.

==> 4Num_Example/parabola_convergence/phase1_c_large_old.tex <==
\subsubsection{Convergence when $c^3$ dominates $cd\kappa$}
\label{sec:4Num-cvgphase1-c-large}
From \cref{sec:4Num-cd-dynamics} we have 
\begin{equation}
\begin{split}
    c'' =&\ c - 16c^3 + 8cd\kappa + \Delta(K_1, c^4) + \Delta(K_2, c^2d\kappa) + \Delta(K_3, cd^2\kappa^2) + \Delta(K_4, c^3\kappa^3) + \Delta(K_5, c\kappa^5),\\
    d'' =&\ d - 4c^2\kappa^3 + \Delta(M_1, c^3\kappa^3) + \Delta(M_2, c^2d\kappa^4) + \Delta(M_3, c^2\kappa^7) + \Delta(M_4, \kappa^{12}).
\end{split}
\end{equation}
Where we set the corresponding absolute constants for the $\Delta$ expressions be $K_1\dots K_5$ for $c''$ and $M_1\dots M_4$ for $d''$ \znote{not rigorous currently, will modify}.
We want to consider the regime such that $|c''| \leq \abs{c} - \abs{c^3}$ when $d > 0$. By triangular inequality, a straightforward setting is just
\begin{equation}
\begin{cases}
    \abs{c^3} &> \abs{cd\kappa}\\
    \abs{c^3} &> \abs{K_1c^4}\\
    \abs{c^3} &> \abs{K_2c^3d\kappa}\\
    \abs{c^3} &> \abs{K_3cd^2\kappa^2}\\
    \abs{c^3} &> \abs{K_4c^3\kappa^3}\\
    \abs{c^3} &> \abs{K_5c\kappa^5}\\
\end{cases}\Rightarrow
\begin{cases}
    \abs{c} > \sqrt{d\kappa} & (1)\\
    \abs{c} < K_1^{-1} & (2)\\
    d < (K_2\kappa)^{-1} & (3)\\
    \abs{c} > \sqrt{K_3}d\kappa & (4)\\
    \kappa < K_4^{-\frac13} & (5)\\
    \abs{c} > \sqrt{K_5\kappa^5} & (6)
\end{cases}
\end{equation}

When setting $d < (K_3 \kappa)^{-1}$, (1) implies (4) since
\begin{equation}
    d < (K_3 \kappa)^{-1}
    \Rightarrow
    K_3d\kappa < 1
    \Rightarrow
    K_3d^2\kappa^2 < d\kappa
    \Rightarrow
    \sqrt{K_3}d\kappa < \sqrt{d\kappa}.
\end{equation}

When setting $d > K_5\kappa^4$ (1) implies (6) since
\begin{equation}
    d > K_5\kappa^4
    \Rightarrow
    \sqrt{d\kappa} > \sqrt{K_5\kappa^5}.
\end{equation}

Thus reorganizing the inequalities, we know that $|c''| \leq |c| - |c^3|$ holds when
\begin{equation}
\begin{split}
    \kappa & \in (0, K_4^{-\frac13})\\
    d & \in (K_5\kappa^4, \min\cbr{(K_2\kappa)^{-1}, (K_3\kappa)^{-1}})\\
    c & \in (\sqrt{dk}, K_1^{-1})
\end{split}
\label{eqn:4Num-ccube-dominate-condition}
\end{equation}
% $\kappa < K_4^{-\frac13}$, $d \in(K_5\kappa^4, \min\cbr{(K_2\kappa)^{-1}, (K_3\kappa)^{-1}})$, and $c\in(\sqrt{dk}, K_1^{-1})$, $|c''| \leq |c| - |c^3|$.

To show the convergence is fast with respect to $d$, we also want to upper bound the movement of $d$. In order for $d'' > d - 8c^2\kappa^3$, by triangle inequality it is sufficient that 
\begin{equation}
\begin{cases}
    \abs{c^2\kappa^3} > M_1\abs{c^3\kappa^3}\\
    \abs{c^2\kappa^3} > M_2\abs{c^2d\kappa^4}\\
    \abs{c^2\kappa^3} > M_3\abs{c^2\kappa^7}\\
    \abs{c^2\kappa^3} > M_4\abs{\kappa^{12}}
\end{cases}
\Rightarrow
\begin{cases}
    \abs{c} < M_1^{-1} & (1)\\
    d < (M_2\kappa)^{-1} & (2)\\
    \kappa < M_3^{-\frac14} & (3)\\
    \abs{c} > M_4\kappa^{\frac92} & (4)\\
\end{cases}
\end{equation}
Reorganizing the inequalities we have $d'' > d - 8c^2\kappa^2$ when
\begin{equation}
\begin{split}
    \kappa & \in (0, M_3^{-\frac14}),\\
    d & \in (0, (M_2\kappa)^{-1}),\\
    c & \in (M_4\kappa^{\frac92}, M_1^{-1}).
\end{split}
\label{eqn:4Num-dmovement-dominate}
\end{equation}
Note that with the bound of $4c^2\kappa^2$ over the $\Delta$ terms of $d''$, we also have $d'' = d - 4c^2\kappa^2 + \Delta(4, c^2\kappa^2) < d$, which means $d''$ is monotonically decreasing.
Combining \cref{eqn:4Num-ccube-dominate-condition} and \cref{eqn:4Num-dmovement-dominate} and setting the additional constraint $d>M_4^2\kappa^8$ to ensure $\sqrt{d\kappa} > M_4\kappa^\frac92$, we have the region
\begin{equation}
\begin{split}
    \kappa & \in (0, \min\scbr{K_4^{-\frac13}, M_3^{-\frac15}}),\\
    d & \in (\max\scbr{M_4^2\kappa^8, K_5\kappa^4}, \min\cbr{(M_2\kappa)^{-1}, (K_2\kappa)^{-1}, (K_3\kappa)^{-1}}),\\
    c & \in (\sqrt{d\kappa}, \min\scbr{M_1^{-1}, K_1^{-1}}).
\end{split}
\label{eqn:4Num-cvgphase1-above-condition}
\end{equation}
Now we are ready to analyze the two step dynamics with 
\begin{equation}
    |c''| < |c| - |c^3|,\qquad d'' > d - 8c^2\kappa^2.
    \label{eqn:4Num-cvgphase1-largec-dynamics}
\end{equation}
For $t\in\NN$, let $(c_t, d_t)$ denote $c$ and $d$ after the $t$-th two step update with step size $\eta=\kappa^2$ from initialization $(c_1, d_1)$.

\begin{lemma}[Convergence to near parabola from large $c$]
    For all $c_1, d_1, \kappa$ satisfying \cref{eqn:4Num-cvgphase1-above-condition}, with the additional constraint of $|c_1|\leq \frac12$,  $d_1 > 9\kappa^3-32\log(\kappa)\kappa^3$ and $\kappa < \min\scbr{K_5^{-1}, M_4^{-\frac13}}$, there exists some $t < (d_1\kappa)^{-1}$ such that $d_t > d_1-8(\kappa^3-4\log(\kappa)\kappa^3)$ 
    % and $|c_t| \in (\sqrt{d\kappa}, 2\sqrt{d\kappa})$.
    and $|c_t| < 2\sqrt{d\kappa}$. \znote{will see what is required by the parabola, could potentially be stronger ($|c_t| \in (\sqrt{d\kappa}, 2\sqrt{d\kappa})$)}
    \label{lemma:4Num-cvgphase1-largec}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:4Num-cvgphase1-largec}]
First note that within the valid region, both $|c|$ and $d$ are monotonically decreasing.
With the additional constraint of $\kappa < \min\scbr{K_5^{-1}, M_4^{-\frac13}}$, we have $\kappa^3 > \max\scbr{M_4^2\kappa^9, K_5\kappa^4}$. Thus as long as $d_t > \kappa^3$ and $c_t > \sqrt{d_t\kappa}$, we have $d_{t+1} > d_t - 8c_t^2\kappa^3$ and $|c_{t+1}| < |c_t| - |c_t^3|$. Now we will prove the claim with induction.

Consider the inductive hypothesis for $t\in\NN$ that if $c_t > \sqrt{d\kappa}$, $|c_t|< t^{-\frac12}$ and $d_t > \kappa^3$. When $t=1$, the base case holds trivially. Now we show the inductive step.

We first upper bound $c_t$. Since $(c_t, d_t)$ are in the valid region for the dynamics described by \cref{eqn:4Num-cvgphase1-largec-dynamics}, according to the inductive hypothesis,
$|c_{t+1}| < |c_t| - |c_t^3|$.
Consider $f(x) = x^{-\frac12}$, we have $f'(x) = -\frac12x^{-\frac32} = -\frac12 f(x)^3$ and $f''(x) = \frac34x^{-\frac52}$. Note that $f''(x) > 0$ for all $x > 0$. Thus by a first order Taylor expansion around $x=t$ we have $f(t+1) > f(t) - \frac12 f(t)^3$. Combined with $|c_{t+1}| < |c_t| - |c_t^3|$, it follows \begin{equation}
\begin{split}
    f(t+1) - c_{t+1} \geq&\ f(t) - \frac12f(t)^3 - c_t + c_t^3\\
    =&\ (f(t)-c_t) - \frac12\srbr{c_t^3 - f(t^3)} + \frac12 c_t^3\\
    \geq&\ (f(t)-c_t) - \frac12(c_t-f(t))(c_t^2 + c_t f(t) + f(t)^2)\\
    =&\ (f(t) - c_t)\rbr{1-\frac12\rbr{c_t^2+c_tf(t)+f(t)^2}}.
\end{split}
\end{equation}
Since $f(t)\leq 1$ and $c_t<\frac12$
% \znote{tbc: might need to be more careful with $c$ when it swaps sign}
for all $t\geq1$, we have  $c_t^2+c_tf(t)+f(t)^2 < 2$, and $\rbr{1-\frac12\rbr{c_t^2+c_tf(t)+f(t)^2}} > 0$. Since $c_t < t^{-\frac12} = f(t)$ by the induction hypothesis, $f(t+1) - c_{t+1} > 0$, which implies $c_{t+1}<(t+1)^{-\frac12}$.
% If there is some $\hat t\in\NN$ such that $c_{\hat{t}+1} < \frac32\sqrt{d\kappa}$, consider the smallest such $\hat t$ and claim that $|c_{\hat{t}}|\in (\frac32\sqrt{d\kappa}, 2\sqrt{d\kappa})$. Since $|c|$ is monotonically decreasing, assume toward contradiction that $c_{\hat{t}} \geq 2\sqrt{d\kappa}.$ Then $|c_{\hat{t}}| - |c_{\hat{t}+1}| > \frac12\sqrt{d\kappa}$
On the other side of $c$, if there exists some $\hat t\in\NN$ such that $c_{\hat{t}+1} < \sqrt{d\kappa}$, then $c_t < 2\sqrt{d\kappa}$, for which case the lemma directly holds and we terminate the induction.

Now we consider the movement of $d$. Since we have shown above that $c_t < f(t)$ for all $t\in\NN$ until $(c,d)$ leaves the region, the total movement of $d$ until time $t$, namely $d_1 - d_t$, can be bounded as follows:
\begin{equation}
\begin{aligned}
d_1 - d_t \leq \sum_{\tau=1}^t8c_\tau^2\kappa^3\leq 8\kappa^3\sum_{\tau=1}^tf(\tau)^2 = 8\kappa^3\sum_{\tau=1}^t\frac1\tau \leq 8\kappa^3\rbr{1+\int_1^t\frac1\tau d\tau} = 8\kappa^3(1+\log(t)).
\end{aligned}
\end{equation}
Since we consider $t$ up to $(d_1\kappa)^{-1}$ and $d_1 > \kappa^3$, we have $\log(t) = \log((d_1\kappa)^{-1})\leq \log(\kappa^{-4}) = -4\log(\kappa)$. Thus $d_0-d_t < 8\kappa^3(1-4\log(\kappa)).$ Since we required $d_0 > 9\kappa^3 - 32\kappa^3\log(\kappa)$, $d_t > 9\kappa^3 - 32\kappa^3\log(\kappa) - 8\kappa^3(1-4\log(\kappa)) = \kappa^3$.
Thus the induction will hold until either $|c_t|$ leaves the region from below or $t\geq \lceil(d\kappa)^{-1}\rceil.$

Since under the inductive hypothesis we have $c_{t+1} < (t+1)^{-\frac12}$ and $d_{t+1} > \kappa^3$, by induction we have $c_t < t^{-\frac12}$ for all $\hat t\in\NN$ 
\znote{need to be more careful when dealing with the ``early termination''}. Thus there exists some $t < \frac14(d\kappa)^{-1}$ such that $c_t < \srbr{\frac14(d\kappa)^{-1}}^{-\frac12} = 2\sqrt{d\kappa},$ which completes the proof.
\end{proof}



==> 4Num_Example/parabola_convergence/phase1_c_small_old.tex <==
\subsubsection{Convergence when $cd\kappa$ dominates $c^3$}
\label{sec:4Num-cvgphase1-c-small}
In this section we follow the same notation as in \cref{sec:4Num-cvgphase1-c-large}.
Recall that
\begin{equation}
\begin{split}
    c'' =&\ c - 16c^3 + 8cd\kappa + \Delta(K_1, c^4) + \Delta(K_2, c^2d\kappa) + \Delta(K_3, cd^2\kappa^2) + \Delta(K_4, c^3\kappa^3) + \Delta(K_5, c\kappa^5),\\
    d'' =&\ d - 4c^2\kappa^3 + \Delta(M_1, c^3\kappa^3) + \Delta(M_2, c^2d\kappa^4) + \Delta(M_3, c^2\kappa^7) + \Delta(M_4, \kappa^{12}).
\end{split}
\end{equation}
We want to consider the regime such that $|c''| > \abs{c} + \abs{cd\kappa}$ when $d > 0$. By triangular inequality, a straightforward setting is just
\begin{equation}
\begin{cases}
    \abs{cd\kappa} &> \abs{8c^3}\\
    \abs{cd\kappa} &> \abs{K_1c^4}\\
    \abs{cd\kappa} &> \abs{K_2c^3d\kappa}\\
    \abs{cd\kappa} &> \abs{K_3cd^2\kappa^2}\\
    \abs{cd\kappa} &> \abs{K_4c^3\kappa^3}\\
    \abs{cd\kappa} &> \abs{K_5c\kappa^5}\\
\end{cases}\Rightarrow
\begin{cases}
    \abs{c} < \frac{1}{2\sqrt{2}}\sqrt{d\kappa} & (1)\\
    \abs{c} < (K_1 d\kappa)^{\frac13} & (2)\\
    \abs{c} < K_2^{-\frac12} & (3)\\
    d < (K_3\kappa)^{-1} & (4)\\
    \abs{c} < K_4^{-\frac12}\sqrt{d} \kappa^{-1} & (5)\\
    d > K_5\kappa^4 & (6)
\end{cases}
\end{equation}

When setting $d < 512 K_1^2\kappa^{-1}$, $(1)$ implies $(2)$ since 
\begin{equation}
    \frac{1}{512}d\kappa < K_1^2
    \Rightarrow
    \rbr{\frac{1}{2\sqrt{2}}}^6d^3\kappa^3 < K_1^2d^2\kappa^2
    \Rightarrow
    \frac{1}{2\sqrt{2}}\sqrt{d\kappa} < (K_1d\kappa)^{\frac13}.
\end{equation}
Note that since we only consider the case with $d < 1$, this bound is vacuous as $\kappa < 0.1$ and $K_1 > 1$.

When setting $d < 8(K_2\kappa)^{-1}$, $(1)$ implies $(3)$ since
\begin{equation}
    d < 8(K_2\kappa)^{-1}
    \Rightarrow
    \frac18 d\kappa < K_2^{-1}
    \Rightarrow
    \frac{1}{2\sqrt{2}}\sqrt{d\kappa} < K_2^{-\frac12}.
\end{equation}

When setting $\kappa < 2K_4^{-\frac13}$, $(1)$ implies $(5)$ since
\begin{equation}
    \kappa < 2K_4^{-\frac13}
    \Rightarrow
    \kappa < \rbr{2\sqrt{2} K_4^{-\frac12}}^{\frac23}
    \Rightarrow
    \kappa^{\frac32} < 2\sqrt{2} K_4^{-\frac12}
    \Rightarrow
    \frac{1}{2\sqrt{2}}\sqrt{d\kappa} < K_4^{-\frac12}\sqrt{d}\kappa^{-1}.
\end{equation}

Thus reorganizing the inequalities, we know that $|c''| \geq |c| + |cd\kappa|$ holds when
\begin{equation}
\begin{split}
    \kappa & \in (0, 2K_4^{-\frac13})\\
    d & \in (K_5\kappa^4, \min\cbr{8(K_2\kappa)^{-1}, (K_3\kappa)^{-1}, 512 K_1^2\kappa^{-1}})\\
    c & \in (0, \frac{1}{2\sqrt{2}}\sqrt{d\kappa})
\end{split}
\label{eqn:4Num-cdkappa-dominate-condition}
\end{equation}
% $\kappa < K_4^{-\frac13}$, $d \in(K_5\kappa^4, \min\cbr{(K_2\kappa)^{-1}, (K_3\kappa)^{-1}})$, and $c\in(\sqrt{dk}, K_1^{-1})$, $|c''| \leq |c| - |c^3|$.

Same as in \cref{sec:4Num-cvgphase1-c-large}, we have $d'' > d - 8c^2\kappa^2$ and $d''\leq d$ when
\begin{equation}
\begin{split}
    \kappa & \in (0, M_3^{-\frac14}),\\
    d & \in (0, (M_2\kappa)^{-1}),\\
    c & \in (M_4\kappa^{\frac92}, M_1^{-1}).
\end{split}
\label{eqn:4Num-dmovement-dominate-RESTATE}
\end{equation}
Combining \cref{eqn:4Num-cdkappa-dominate-condition} and \cref{eqn:4Num-dmovement-dominate-RESTATE}, and set the extra constraint of $d < 8\kappa^{-1}M_1^{-2}$ so that $\frac{1}{2\sqrt{2}}\sqrt{d\kappa} < M_1^{-1},$ we have the region
\begin{equation}
\begin{split}
    \kappa & \in (0, \min\scbr{2K_4^{-\frac13}, M_3^{-\frac14}}),\\
    d & \in (K_5\kappa^4, \min\cbr{8(\kappa M_1^2)^{-1}, (M_2\kappa)^{-1}, 8(K_2\kappa)^{-1}, (K_3\kappa)^{-1}, 512 K_1^2\kappa^{-1}}),\\
    c & \in (M_4\kappa^5, \frac{1}{2\sqrt{2}}\sqrt{d\kappa}).
\end{split}
\label{eqn:4Num-cvgphase1-small-condition}
\end{equation}
Now we are ready to analyze the two step dynamics with 
\begin{equation}
    |c''| > |c| + |cd\kappa|,\qquad d'' > d - 8c^2\kappa^2.
    \label{eqn:4Num-cvgphase1-largec-dynamics}
\end{equation}
Similar to \cref{sec:4Num-cvgphase1-c-large}, for $t\in\NN$, let $(c_t, d_t)$ denote $c$ and $d$ after the $t$-th two step update with step size $\eta=\kappa^2$ from initialization $(c_1, d_1)$.

\begin{lemma}[Convergence to near parabola from small $c$]
    For all $c_1, d_1, \kappa$ satisfying \cref{eqn:4Num-cvgphase1-small-condition}, with the additional constraint of $d_1 > 16\kappa^3$, there exists some $t < \srbr{\frac12\log(d_1\kappa)-\log(c_1)}\srbr{1 + \frac18\kappa^{-4}}$ such that $d_t > d_1-\frac14\sqrt{d_1}\kappa^{\frac32}$ 
    % and $|c_t| \in (\sqrt{d\kappa}, 2\sqrt{d\kappa})$.
    and $|c_t| > \frac14\sqrt{d\kappa}$. \znote{will see what is required by the parabola}
    \label{lemma:4Num-cvgphase1-smallc}
\end{lemma}
\begin{proof}[Proof of Lemma \cref{lemma:4Num-cvgphase1-smallc}]
First note that within the valid region, $d$ is monotonically decreasing and $|c|$ is monotonically increasing, in particular recall that $d_{t+1} > d_t - 8c_t^2\kappa^3$ and $|c_{t+1}| > |c_t| + |c_td_t\kappa|$.

Observe that when $d$ is not too small, the movement of $c$ in the valid region is significantly larger than the movement of $d$. Formally, when $d_t > 8\kappa^3$,
\begin{equation}
\begin{aligned}
    \frac{c_{t+1} - c_t}{d_{t} - d_{t+1}} > 
    \frac{|c_t|d_t\kappa}{8c_t^2\kappa^3} =&\ \frac{1}{|c_t|}\frac{d_t}{8\kappa^2}\\
    >&\ \frac{2\sqrt{2}}{\sqrt{d_t\kappa}}\frac{d_t}{8\kappa^2} &(\text{since}\ c < \frac{1}{2\sqrt{2}}\sqrt{d\kappa})\\
    =&\ \frac{1}{2\sqrt{2}}\frac{\sqrt{d_t}}{\kappa^{\frac52}}\\
    >& \frac{2\sqrt{2}\kappa^{\frac32}}{2\sqrt{2}\kappa^{\frac52}} = \kappa^{-1}. & (\text{since}\ d_t > 8\kappa^3)
\end{aligned}
\end{equation}

We will now prove the claim with induction. 
Consider the inductive hypothesis for $t > 1$ that if $c_t < \frac14\sqrt{d\kappa}$, $\srbr{|c_t| - |c_1|}/\srbr{d_1 - d_t} > \frac1\kappa.$ The base case holds trivially as $d_1 > 16\kappa^3$. 
For the inductive step, if $c_t \geq \frac14\sqrt{d\kappa}$, the lemma directly holds \znote{need to be a bit more careful to show that the last movement of $d$ is small, will add later}.

When $|c_t| < \frac14\sqrt{d\kappa}$, the inductive hypothesis gives $\srbr{|c_t| - |c_1|}/\srbr{d_1 - d_t} > \frac1\kappa$. By the mediant inequality, in order to show $\srbr{|c_{t+1}| - |c_1|}/\srbr{d_1 - d_{t+1}} > \frac1\kappa$, we only need to show $\srbr{|c_{t+1}| - |c_t|}/\srbr{d_{t} - d_{t+1}} > \frac1\kappa$, which is true when $d_{t} > 8\kappa^3$.
Note that $|c_t| - |c_1| \leq |c_t| < \frac14\sqrt{d_t\kappa} < \frac14\sqrt{d_1\kappa}$ where last inequality holds since $d_t$ is monotonically decreasing. Plugging in the inductive hypothesis we have $d_1 - d_t < \kappa(|c_t| - |c_1|) = \frac14\sqrt{d_1}\kappa^{\frac32}.$ Hence $d_t > d_1 - \frac14\sqrt{d_1}\kappa^{\frac32} = \sqrt{d_1}(\sqrt{d_1}-\frac14\kappa^{\frac32})$. Since $d_1 > 16\kappa^3$, $\sqrt{d_1} > 4\kappa^{\frac32}$, and thus $d_t > \sqrt{d_1}(\sqrt{d_1}-\frac14\kappa^{\frac32}) > 4\kappa^{\frac32}(4\kappa^{\frac32}-\frac14\kappa^{\frac32}) > 8\kappa^3$, this completes the induction.

Now we only need to show that $c_t$ will exceed $\frac14\sqrt{d\kappa}$ in finite time. Note that in this regime $c_t$ has multiplicative update $|c_{t+1}| = |c_t| + |c_td_t\kappa| = |c_t|(1+d_t\kappa)$. From above we know that $d_t > 8\kappa^3$ for all $t$ such that $|c_t| < \frac14\sqrt{d\kappa}$, so $|c_{t+1}| \geq |c_{t}|(1+8\kappa^4).$ Therefore for $c$ to increase from $c_1$ to $\frac14\sqrt{d_t\kappa}$ for some $t$, the number of steps is at most
\begin{equation}
\begin{aligned}
    t =&\ \frac{\log\rbr{\frac14\sqrt{d_t\kappa}/c_1}}{\log\rbr{1+8\kappa^4}}\\
    \leq&\ \frac{\log\rbr{\frac14\sqrt{d_1\kappa}/c_1}}{\log\rbr{1+8\kappa^4}} & (\text{since}\ d_t\  \text{is monotonically decreasing})\\
    \leq& \rbr{\frac12\log(d_1\kappa)-\log(c_1)}\frac{1+8\kappa^4}{8\kappa^4} & (\text{since}\ \log(1+x)\geq x/(1+x))\\
    \leq& \rbr{\frac12\log(d_1\kappa)-\log(c_1)}\rbr{1 + \frac18\kappa^{-4}}.
\end{aligned}
\end{equation}

This completes the proof for this lemma.
\end{proof}



==> 4Num_Example/parabola_convergence/phase1_stay_old.tex <==
\subsubsection{$c$ stays in $(\frac14\sqrt{d\kappa}, 2\sqrt{d\kappa})$ as $d$ decreases when $d$ is not too small}
After showing that $c$ will enter $(\frac14\sqrt{d\kappa}, 2\sqrt{d\kappa})$, we now show that it will not leave this region unless $d$ is very small. To do so, we first determine a regime in which we can effectively bound the two-step movement of $c$.

\input{4Num_Example/parabola_convergence/phase1_stay_regime.tex}

With the two-step movement of $c$ bounded above, we may proceed to state the lemma that guarantees $c$ will not leave $(\frac14\sqrt{d\kappa}, 2\sqrt{d\kappa})$ unless $d$ is very small.

\begin{lemma}
\label{lemma:4Num-phase1-stay}
For any $\kappa$ and initialization $c_1, d_1$ satisfying
\begin{equation}
\begin{split}
    \kappa &< \frac{1}{16}K^{-1},\\
    d_1&\in (2\kappa^{\frac52}, \min\scbr{1, \frac14K^{-2}\kappa^{-1}}),\\
    |c_1|&\in (\frac14\sqrt{d_1\kappa}, 2\sqrt{d_1\kappa}).
\end{split}
\end{equation}
There exists some $T \leq \frac{32}{3}d_1\kappa^{-\frac{13}{2}}$ such that $d_T\in (\frac32\kappa^{\frac52}, 2\kappa^{\frac52})$ and for all $t < T$, $c_t\in (\frac14\sqrt{d_t\kappa}, 2\sqrt{d_t\kappa})$. 
\end{lemma}

\begin{proof}[Proof of \cref{lemma:4Num-phase1-stay}]
First we check that the region defined is not empty. This is true since given $\kappa < \frac{1}{16}K^{-1}$, we have $\frac14K^{-2}\kappa^{-1} > 4K^{-1} > 2K^{-\frac52} > 2\kappa^{\frac52}$.

Now claim that there exists some $\hat t \leq \frac{32}{3}d_1\kappa^{-\frac{13}{2}} + 1$ such that $d_{\hat{t}} < \frac32\kappa^{\frac52}$ and for all $t < \hat t$, $d_t\in (\frac32\kappa^{\frac52}, d_1]$ and $c_t\in (\frac14\sqrt{d_t\kappa}, 2\sqrt{d_t\kappa}).$ To prove so we consider the inductive hypothesis 
\begin{center}
$P(k)$: $d_k \in (\frac32\kappa^{\frac52}, d_1 - \frac{3}{32}(k-1)\kappa^{\frac{13}{2}}]$ and $|c_k| \in (\frac14\sqrt{d_k\kappa}, 2\sqrt{d_k\kappa})$.
\end{center}
Assume that $P(k)$ holds for some $k$. Since $d_k < d_1 < \frac14K^{-2}\kappa^{-1}$, we have $|c_k| < 2\sqrt{d_k\kappa} < 2\sqrt{\frac14K^{-2}\kappa^{-1}\kappa} = K^{-1}.$ With $\kappa < \frac{1}{16}K^{-1}$ and $d_k < d_1 < \frac{1}{4}K^{-2}\kappa^{-1}$, we have $\kappa,c_k,d_k$ satisfying \cref{cond:4Num-d-delta-regime} and \cref{cond:4Num-c-movement-bounded}.
Thus $d_{k+1} < d_{k}-c_k^2\kappa^3$, $d_{k+1} > d_{k}-8c_k^2\kappa^3$ (by \cref{lemma:4Num-d-2step-movement-regime}), and $|c_{k+1} - c_k| < \frac{1}{16}\sqrt{d_k\kappa}$ (by \cref{lemma:4Num-bounded-2step-c-movement}).
Observe that since $d_{k+1} > d_{k}-8c_k^2\kappa^3$, 
\begin{equation}
\begin{aligned}
\label{eqn:4Num-stay-dk-decrease-upperbound}
2\sqrt{d_{k+1}\kappa} &> 2\sqrt{(d_{k}-8c_k^2\kappa^3)\kappa}\\
&> 2\sqrt{(d_k - 8(4d_k\kappa)\kappa^3)\kappa} & (\text{since}\ c_k < 2\sqrt{d_k\kappa})\\
&= 2\sqrt{(d_k\kappa)(1-32\kappa^4)}\\
&= 2\sqrt{1-32\kappa^4}\sqrt{d_k\kappa}
\end{aligned}
\end{equation}
Note that with $\kappa < \frac{1}{16}K^{-1}$ where we assume $K > 128$, we have $\sqrt{1-32\kappa^4} > 0.99$ and hence $\sqrt{d_{k+1}\kappa} > 0.99\sqrt{d_k\kappa}.$
Now we will show that $c_{k+1}$ will not leave $(\frac14\sqrt{d_{k+1}\kappa}, 2\sqrt{d_{k+1}\kappa})$. There are three cases to consider:
\begin{enumerate}
\item
When $|c_k| \in (\sqrt{d_k\kappa}, 2\sqrt{d_k\kappa})$, along with $|c_k| < K^{-1}$ we have \cref{cond:4Num-c-large-regime} satisfied and thus $|c_{k+1}| < |c_{k}|(1 - c_{k}^2)$ by \cref{lemma:4Num-c-large-regime}. Since $\kappa < \frac{1}{16}K^{-1} < \frac{1}{2048}$, we have $\kappa^{\frac14} < \frac{\sqrt{3}}{8} = \frac{1}{4\sqrt{2}}\sqrt{3/2}$, and thus $\sqrt{3/2}\kappa^{\frac74} > 4\sqrt{2}\kappa^2$.

Moreover, since $d_k > \frac32\kappa^{\frac52}$, we have $|c_k| > \sqrt{d_k\kappa} > \sqrt{3/2}\kappa^{\frac74} > 4\sqrt{2}\kappa^2$. Squaring both sides we have $c_k^2 > 32\kappa^4$. Hence $1-32\kappa^4 > 1-c_k^2 > 1-2c_k^2 + c_k^4 = (1-c_k^2)^2$. The last inequality holds since $c_k^2 > c_k^4$ as $|c_k| < 1$. Now taking the square root on both sides we have $1-c_k^2 < \sqrt{1-32\kappa^4}.$
Since $|c_k| < 2\sqrt{d_k\kappa}$, combining with \cref{eqn:4Num-stay-dk-decrease-upperbound} and $1-c_k^2 < \sqrt{1-32\kappa^4}$ we have $|c_{k+1}| < 2\sqrt{d_k\kappa}(1-c_k^2) < 2\sqrt{1-32\kappa^4}\sqrt{d_k\kappa} < 2\sqrt{d_{k+1}\kappa}$, which gives the desired upper bound to $|c_{k+1}|$.

Now we prove the lower bound for $|c_{k+1}|$. Since we know $|c_{k+1} - c_k| < \frac{1}{16}\sqrt{d_k\kappa}$, by triangle inequality, $|c_k| > \sqrt{d\kappa}$ implies $|c_{k+1}| > \frac{15}{16}\sqrt{d_{k}\kappa} > \frac{1}{4}\sqrt{d_{k}\kappa} > \frac14\sqrt{d_{k+1}\kappa}$

\item
When $|c_k| \in [\frac{1}{2\sqrt{2}}\sqrt{d_k\kappa}, \sqrt{d_k\kappa}]$, since $|c_{k+1} - c_k| < \frac{1}{16}\sqrt{d_k\kappa}$, by triangle inequality we have $|c_{k+1}| \in [(\frac{1}{2\sqrt{2}}-\frac{1}{16})\sqrt{d_k\kappa}, \frac{17}{16}\sqrt{d_k\kappa}]$. Since $(\frac{1}{2\sqrt{2}}-\frac{1}{16})\sqrt{d_k\kappa} > \frac{1}{4}\sqrt{d_k\kappa} > \frac{1}{4}\sqrt{d_{k+1}\kappa}$ and $\frac{17}{16}\sqrt{d_k\kappa} < 2\sqrt{d_{k+1}\kappa}$ as $\sqrt{d_{k+1}\kappa} > 0.99\sqrt{d_k\kappa}$, we have $|c_{k+1}| \in (\frac{1}{4}\sqrt{d_k\kappa}, 2\sqrt{d_k\kappa})$.

\item
When $|c_k| \in (\frac14\sqrt{d_k\kappa}, \frac{1}{2\sqrt{2}}\sqrt{d_k\kappa})$, along with $|c_k| < K^{-1}$ we have \cref{cond:4Num-c-small-regime} satisfied, and thus $|c_{k+1}| > |c_k| + |c_kd_k\kappa| > |c_k|$. Since $\sqrt{d_{k+1}\kappa} < \sqrt{d_k\kappa}$, $|c_{k+1}| > \frac14\sqrt{d_{k+1}\kappa}$.

On the other side, since $|c_{k+1}-c_k| < \frac{1}{16}\sqrt{d_k\kappa}$, and $|c_k| < \frac{1}{2\sqrt{2}}\sqrt{d_k\kappa}$, by triangle inequality we have $|c_{k+1}| < (\frac{1}{16} + \frac{1}{2\sqrt{2}})\sqrt{d_k\kappa} < 2\sqrt{d_{k+1}\kappa}.$ The last step holds since $\sqrt{d_{k+1}\kappa} > 0.99\sqrt{d_k\kappa}$.
\end{enumerate}

Summarizing the three cases, we know that $c_{k+1}\in (\frac14\sqrt{d_{k+1}\kappa}, 2\sqrt{d_{k+1}\kappa}).$

By the assumption of $P(k)$ we also have $d_k > \frac32\kappa^{\frac52}$ and $d_k < d_1 - \frac{3}{32}(k-1)\kappa^{\frac{13}{2}}$. Since we know $c_k > \frac14\sqrt{d_k\kappa}$, we have $c_k^2\kappa^3 > \frac{1}{16}d_k\kappa^4 > \frac{3}{32}\kappa^{\frac{13}{2}}.$ Thus $d_{k+1} < d_{k} - c_k^2\kappa^3 < d_k - \frac{3}{32}\kappa^{\frac{13}{2}} < d_1 - \frac{3}{32}k\kappa^{\frac{13}{2}}$. Therefore unless $c_{k+1} < \frac{3}{2}\kappa^{\frac52}$, $P(k+1)$ holds. Note that there must be some $t$ such that $d_t < \frac32\kappa^{\frac52}$ since when $t > \frac{32}{3}d_1\kappa^{-\frac{13}{2}} + 1$, $d_1 - \frac{3}{32}(t-1)\kappa^{\frac{13}{2}} < 0.$
We induct on $k$ from $1$, the base case holds by the initialization of $c_1$ and $d_1$. Let $\hat t$ be the smallest $t$ such that $d_t < \frac32\kappa^{\frac52}$, at which we terminate the induction. Then for all $t < \hat t$, $d_t\in (\frac32\kappa^{\frac52}, d_1]$ and $c_t\in (\frac14\sqrt{d_t\kappa}, 2\sqrt{d_t\kappa}).$

By definition of $\hat t$ we know $P(\hat t - 1)$ holds. Let $T = \hat t -1$, then from above we have $d_T > \frac32\kappa^{\frac52}$, $c_T < K^{-1}$, and $d_{\hat t} > d_T - 7c_T^2\kappa^3$. Therefore $d_T < d_{\hat t} + 7c_T^2\kappa^3 < \frac32\kappa^{\frac52} + 7K^{-1}\kappa^3 < 2\kappa^{\frac52}$. The last inequality holds since $\kappa < 1$ and we assume $K > 128$. Since $P(t)$ holds for all $t \leq T$ by definition of $T$, $c_t\in (\frac14\sqrt{d_t\kappa}, 2\sqrt{d_t\kappa})$ for all $t \leq T$. Combining with $d_T < 2\kappa^{\frac52}$ and $d_T > \frac32\kappa^{\frac52}$ completes the proof.
\end{proof}



==> 4Num_Example/parabola_convergence/phase2_parabola_convergence.tex <==
\subsubsection{Convergence when $cd\kappa$ dominates $c^3$}
\label{sec:4Num-cvgphase2}
In this section we follow the same notation as in \cref{sec:4Num-cvgphase1-c-large}.
Recall that
\begin{equation}
\begin{split}
    c'' =&\ c - 16c^3 + 8cd\kappa + \Delta(K_1, c^4) + \Delta(K_2, c^2d\kappa) + \Delta(K_3, cd^2\kappa^2) + \Delta(K_4, c^3\kappa^3) + \Delta(K_5, c\kappa^5),\\
    d'' =&\ d - 4c^2\kappa^3 + \Delta(M_1, c^3\kappa^3) + \Delta(M_2, c^2d\kappa^4) + \Delta(M_3, c^2\kappa^7) + \Delta(M_4, \kappa^{12}).
\end{split}
\end{equation}
We want to consider the regime such that $c''-c$ is both determined by ${c}^3$ and ${cd\kappa}$ when $d > 0$. We prove that the trajectory will eventually converge to a `parabolic region' that is bounded by two parabolas. First we specify the setting where $c^3$ and $cd\kappa$ is dominant in the dynamics. Consider some small constant $\epsilon$.
\begin{equation}
\begin{cases}
    \epsilon\abs{c^3} &> \abs{K_1c^4}\\
    \epsilon\abs{cd\kappa} &> \abs{K_2c^3d\kappa}\\
    \epsilon\abs{cd\kappa} &> \abs{K_3cd^2\kappa^2}\\
    \epsilon\abs{c^3} &> \abs{K_4c^3\kappa^3}\\
    \epsilon\abs{cd\kappa} &> \abs{K_5c\kappa^5}\\
\end{cases}\Rightarrow
\begin{cases}
    \abs{c} < \epsilon / K_1 & (1)\\
    \abs{c} < K_2^{-\frac12}\epsilon^{1/2} & (2)\\
    d < (K_3\kappa)^{-1}\epsilon & (3)\\
    \epsilon < K_4\kappa^{3} & (4)\\
    d > K_5\kappa^4\epsilon^{-1} & (5)
\end{cases}
\label{eqn:4Num-cvgphase2-c-condition}
\end{equation}

In this regime, we have the two step dynamics be bounded by the two expressions:

\begin{equation}
\begin{split}
    c'' >&\ c - (16+2\epsilon)c^3 + (8-3\epsilon)cd\kappa ,\\
    c'' <&\ c - (16-2\epsilon)c^3 + (8+3\epsilon)cd\kappa \\
\end{split}
\end{equation}

Similarly, we specify the regime constraint of $d$ dynamics.
\begin{equation}
\begin{cases}
    \epsilon\abs{c^2\kappa^3} > M_1\abs{c^3\kappa^3}\\
    \epsilon\abs{c^2\kappa^3} > M_2\abs{c^2d\kappa^4}\\
    \epsilon\abs{c^2\kappa^3} > M_3\abs{c^2\kappa^7}\\
    \epsilon\abs{c^2\kappa^3} > M_4\abs{\kappa^{12}}
\end{cases}
\Rightarrow
\begin{cases}
    \abs{c} < M_1^{-1}\epsilon & (1)\\
    d < (M_2\kappa)^{-1}\epsilon & (2)\\
    \kappa < M_3^{-\frac14}\epsilon^{-\frac{1}{4}} & (3)\\
    \abs{c} > M_4^{\frac12}\kappa^{\frac92}\epsilon^{-\frac12} & (4)\\
\end{cases}
\label{eqn:4Num-cvgphase2-d-condition}
\end{equation}
And we have the dynamics:
\begin{equation}
\begin{split}
    d'' >&\ d - (4+4\epsilon)c^2\kappa^3.\\
    d'' <&\ d - (4-4\epsilon)c^2\kappa^3.
\end{split}
\end{equation}
% Combining \cref{eqn:4Num-cdkappa-dominate-condition} and \cref{eqn:4Num-dmovement-dominate-RESTATE}, and set the extra constraint of $d < 8\kappa^{-1}M_1^{-2}$ so that $\frac{1}{2\sqrt{2}}\sqrt{d\kappa} < M_1^{-1},$ we have the region
% \begin{equation}
% \begin{split}
%     \kappa & \in (0, \min\scbr{2K_4^{-\frac13}, M_3^{-\frac14}}),\\
%     d & \in (K_5\kappa^4, \min\cbr{8(\kappa M_1^2)^{-1}, (M_2\kappa)^{-1}, 8(K_2\kappa)^{-1}, (K_3\kappa)^{-1}, 512 K_1^2\kappa^{-1}}),\\
%     c & \in (M_4\kappa^5, \frac{1}{2\sqrt{2}}\sqrt{d\kappa}).
% \end{split}
% \label{eqn:4Num-cvgphase1-small-condition}
% \end{equation}
% Now we are ready to analyze the two step dynamics with 
% \begin{equation}
%     |c''| > |c| + |cd\kappa|,\qquad d'' > d - 8c^2\kappa^2.
%     \label{eqn:4Num-cvgphase1-largec-dynamics}
% \end{equation}
% Similar to \cref{sec:4Num-cvgphase1-c-large}, for $t\in\NN$, let $(c_t, d_t)$ denote $c$ and $d$ after the $t$-th two step update with step size $\eta=\kappa^2$ from initialization $(c_1, d_1)$.

\begin{lemma}[Convergence when near parabola]
    For all $c_1, d_1, \kappa$ satisfying \cref{eqn:4Num-cvgphase2-c-condition} and \cref{eqn:4Num-cvgphase2-d-condition}, with the additional constraint of $d_1 > 16\kappa^3$, there exists some $t < \srbr{\frac12\log(d_1\kappa)-\log(c_1)}\srbr{1 + \frac18\kappa^{-4}}$ such that $d_t > d_1-\frac14\sqrt{d_1}\kappa^{\frac32}$ 
    % and $|c_t| \in (\sqrt{d\kappa}, 2\sqrt{d\kappa})$.
    and $|c_t| > \frac14\sqrt{d\kappa}$. \znote{will see what is required by the parabola}
    \label{lemma:4Num-cvgphase2}
\end{lemma}
\begin{proof}[Proof of Lemma \ref{lemma:4Num-cvgphase1-smallc}]
First note that within the valid region, $d$ is monotonically decreasing and $|c|$ is monotonically increasing, in particular recall that $d_{t+1} > d_t - 8c_t^2\kappa^3$ and $|c_{t+1}| > |c_t| + |c_td_t\kappa|$.

Observe that when $d$ is not too small, the movement of $c$ in the valid region is significantly larger than the movement of $d$. Formally, when $d_t > 8\kappa^3$,
\begin{equation}
\begin{aligned}
    \frac{c_{t+1} - c_t}{d_{t} - d_{t+1}} > 
    \frac{|c_t|d_t\kappa}{8c_t^2\kappa^3} =&\ \frac{1}{|c_t|}\frac{d_t}{8\kappa^2}\\
    >&\ \frac{2\sqrt{2}}{\sqrt{d_t\kappa}}\frac{d_t}{8\kappa^2} &(\text{since}\ c < \frac{1}{2\sqrt{2}}\sqrt{d\kappa})\\
    =&\ \frac{1}{2\sqrt{2}}\frac{\sqrt{d_t}}{\kappa^{\frac52}}\\
    >& \frac{2\sqrt{2}\kappa^{\frac32}}{2\sqrt{2}\kappa^{\frac52}} = \kappa^{-1}. & (\text{since}\ d_t > 8\kappa^3)
\end{aligned}
\end{equation}

We will now prove the claim with induction. 
Consider the inductive hypothesis for $t > 1$ that if $c_t < \frac14\sqrt{d\kappa}$, $\srbr{|c_t| - |c_1|}/\srbr{d_1 - d_t} > \frac1\kappa.$ The base case holds trivially as $d_1 > 16\kappa^3$. 
For the inductive step, if $c_t \geq \frac14\sqrt{d\kappa}$, the lemma directly holds \znote{need to be a bit more careful to show that the last movement of $d$ is small, will add later}.

When $|c_t| < \frac14\sqrt{d\kappa}$, the inductive hypothesis gives $\srbr{|c_t| - |c_1|}/\srbr{d_1 - d_t} > \frac1\kappa$. By the mediant inequality, in order to show $\srbr{|c_{t+1}| - |c_1|}/\srbr{d_1 - d_{t+1}} > \frac1\kappa$, we only need to show $\srbr{|c_{t+1}| - |c_t|}/\srbr{d_{t} - d_{t+1}} > \frac1\kappa$, which is true when $d_{t} > 8\kappa^3$.
Note that $|c_t| - |c_1| \leq |c_t| < \frac14\sqrt{d_t\kappa} < \frac14\sqrt{d_1\kappa}$ where last inequality holds since $d_t$ is monotonically decreasing. Plugging in the inductive hypothesis we have $d_1 - d_t < \kappa(|c_t| - |c_1|) = \frac14\sqrt{d_1}\kappa^{\frac32}.$ Hence $d_t > d_1 - \frac14\sqrt{d_1}\kappa^{\frac32} = \sqrt{d_1}(\sqrt{d_1}-\frac14\kappa^{\frac32})$. Since $d_1 > 16\kappa^3$, $\sqrt{d_1} > 4\kappa^{\frac32}$, and thus $d_t > \sqrt{d_1}(\sqrt{d_1}-\frac14\kappa^{\frac32}) > 4\kappa^{\frac32}(4\kappa^{\frac32}-\frac14\kappa^{\frac32}) > 8\kappa^3$, this completes the induction.

Now we only need to show that $c_t$ will exceed $\frac14\sqrt{d\kappa}$ in finite time. Note that in this regime $c_t$ has multiplicative update $|c_{t+1}| = |c_t| + |c_td_t\kappa| = |c_t|(1+d_t\kappa)$. From above we know that $d_t > 8\kappa^3$ for all $t$ such that $|c_t| < \frac14\sqrt{d\kappa}$, so $|c_{t+1}| \geq |c_{t}|(1+8\kappa^4).$ Therefore for $c$ to increase from $c_1$ to $\frac14\sqrt{d_t\kappa}$ the number of steps $t$ is at most
\begin{equation}
\begin{aligned}
    t =&\ \frac{\log\rbr{\frac14\sqrt{d_t\kappa}/c_1}}{\log\rbr{1+8\kappa^4}}\\
    \leq&\ \frac{\log\rbr{\frac14\sqrt{d_1\kappa}/c_1}}{\log\rbr{1+8\kappa^4}} & (\text{since}\ d_t\  \text{is monotonically decreasing})\\
    \leq& \rbr{\frac12\log(d_1\kappa)-\log(c_1)}\frac{1+8\kappa^4}{8\kappa^4} & (\text{since}\ \log(1+x)\geq x/(1+x))\\
    \leq& \rbr{\frac12\log(d_1\kappa)-\log(c_1)}\rbr{1 + \frac18\kappa^{-4}}.
\end{aligned}
\end{equation}

This completes the proof for this lemma.
\end{proof}



==> 4Num_Example/parabola_convergence/xi_regime_old.tex <==

\begin{lemma}
\label{lemma:4Num-xi-regime}
    For any $\eps < (\delta L_5^{-1})/5$. For all $\kappa, c, d$ satisfying \cref{cond:4Num-1step-dynamics} with the extra constraint of $\kappa < \min\scbr{(\delta L_2^{-1}/10)^{\frac65}, (\delta L_3^{-1}/20)^{\frac13}, \delta L_4^{-1}/5}$, $|d| < 2\kappa^{\frac52}$ and $|c| < (\delta L_1^{-1}/5)^{\frac13}\kappa^{\frac43}$, we have
    \begin{equation}
        \abs{\xi'' - (1-32c^2)\xi} < \delta c^2\kappa^4.
    \end{equation}
\end{lemma}

\begin{proof}[Proof of \cref{lemma:4Num-xi-regime}]
First we check that $\eps = (\delta L_5^{-1})/5 < 0.5$, so \cref{eqn:4Num-xi-remainder} applies. Also note that \cref{cond:4Num-1step-dynamics} are all upper bounds on $\kappa, c, d$, so combining with the additional constraints will define a non-empty regime.

\begin{itemize}
\item 
Given $|c| < (\delta L_1^{-1}/5)^{\frac13}\kappa^{\frac43}$, we have $|c^3| < (\delta L_1^{-1}/5)\kappa^4$ and hence $L_1|c^5| < (\delta /5)c^2\kappa^4$.

\item
Given $\kappa < (\delta L_2^{-1}/10)^{\frac65}$, we have $\kappa^{\frac56} < \delta L_2^{-1}/10$ and hence $2\kappa^{\frac{23}{6}} < L_2^{-1}\kappa^3\delta / 5$. Note that when $|c| < (\delta L_1^{-1}/5)^{\frac13}\kappa^{\frac43}$,  $|c| < \kappa^{\frac43}$. Therefore $|cd| < 2\kappa^{\frac52}\kappa^{\frac43} = 2\kappa^{\frac{23}{6}} < L_2^{-1}\kappa^3\delta/5$. Multiplying $L_2c^2\kappa$ on both sides we have $L_2|c^3d\kappa| < (\delta/5)c^2\kappa^4.$

\item
Given $\kappa < (\delta L_3^{-1}/20)^{\frac13}$, we have $2\kappa^{\frac32} < L_3^{-\frac12}(\delta/5)^{\frac12}$. It follows that $L_3^{-\frac12}(\delta/5)^{\frac12}\kappa > 2\kappa^{\frac52} > d.$ Squaring both sides we have $d^2 < L_3^{-1}(\delta/5)\kappa^2$. Multiplying $<L_3c^2\kappa^2$ on both sides we have $L_3c^2d^2\kappa^2 < (\delta/5)c^2\kappa^4.$

\item
Given $\kappa < (\delta/5)L_4^{-1}$, since $|c| <\kappa^{\frac43} < \kappa$, we have $|c| < (\delta/5)L_4^{-1}$. Multiplying $L_4c^2\kappa^4$ on both sides we have $L_4|c^3\kappa^4| < (\delta/5)c^2\kappa^4$.

\item
Given $\eps < (\delta/5) L_5^{-1}$, multiplying both sides by $L_5c^2\kappa^4$ we have $L_5|\eps c^2\kappa^4| = (\delta/5) c^2\kappa^4$.
\end{itemize}
Combining above we have \begin{equation}
    |R_\xi| < L_1\abs{c^5} + L_2\abs{c^3d\kappa} + L_3\abs{c^2d^2\kappa^2} + L_4\abs{c^3\kappa^4} + L_5\abs{\eps c^2\kappa^4} < \delta c^2\kappa^4.
\end{equation}
Plugging back into \cref{eqn:4Num-xi-remainder} completes the proof.
\end{proof}

==> 4Num_Example/tedious_derivations/d1_lagrange_remainder.tex <==
% \begin{landscape}
\subsubsection{Constant bound on $R_{d}(\kappa)$}
\label{sec:4Num-tediou-d1-remainder}
\znote{will need to change to 13-th order, is there a better way?}
Here we bound the coefficient for the 6-th order Lagrange remainder $R_\delta(\kappa)$ for the expansion
\begin{equation}
    d'\kappa = d\kappa - \frac12\rbr{c^2(1+c)^2(2+c)^2}\kappa^4 + R_d(\kappa)\kappa^5.
\end{equation}
Since $d'\kappa$ is $C^5$ with respect to $\kappa$, we have $R_\delta(\kappa) = \frac{\partial^5 (d'\kappa)}{\partial \kappa^5}(x)/120$ for some $x\in [0,\kappa]$.

Recall that $\kappa < 0.1$ and $c,d\in[-1,1]$. We use the same definition of $\alpha$ and $\rho_1,\dots,\rho_6$ as in \cref{sec:4Num-tediou-delta-remainder}
Moreover, let $\xi = c^2(1+c)^2(2+c)^2$ and $\sigma = \rbr{1-\xi\kappa^4}^{\frac12}$. By doing some tedious calculation we have
\begin{equation}
\begin{split}
\frac{\partial^5 (d'\kappa)}{\partial \kappa^5}(x) =&\ (\alpha+d \kappa)  \rbr{-\frac{3360 \kappa^{15} \xi}{\sigma^9}-\frac{7200 \kappa^{11} \xi}{\sigma^7}-\frac{4680 \kappa^7 \xi}{\sigma^5}-\frac{840 \kappa^3 \xi}{\sigma^3}}\\
&\ + \rbr{5d - \frac{20\kappa^3}{\alpha^3}} \rbr{-\frac{240 \kappa^{12} \xi}{\sigma^7}-\frac{432 \kappa^8 \xi}{\sigma^5}-\frac{204 \kappa^4 \xi}{\sigma^3}-\frac{12 \xi}{\sigma}}\\
&\ + 10 \rbr{-\frac{24 \kappa^9 \xi}{\sigma^5}-\frac{36 \kappa^5 \xi}{\sigma^3}-\frac{12 \kappa  \xi}{\sigma}} \rho_2 + 10 \rbr{-\frac{4 \kappa^6 \xi}{\sigma^3}-\frac{6 \kappa^2 \xi}{\sigma}} \rho_3-\frac{10 \kappa^3 \xi}{\sigma}\rho_4 + \rbr{\sigma-1} \rho_5.
\end{split}
\end{equation}
Since we know from \cref{sec:4Num-tediou-delta-remainder} that with $\kappa < 0.1$, $|\alpha|$ is bounded above by some constant, so $\alpha + d\kappa$, $5d-20\kappa^3/\alpha^3$ are bounded above by some constant independent of $\kappa,c,d$. Since we assume $c\leq 1$, $\xi=c^2(1+c)^2(2+c)^2 \leq 36$.
It follows that $\sigma=\rbr{1-\xi\kappa^4}^{\frac12} \geq \rbr{1-36\times 0.1^4}^{\frac12} > 0.99$. It is also straightforward that $\sigma\leq 1$.

Note that $\frac{\partial^5 (d'\kappa)}{\partial \kappa^5}(x)$ is a finite degree polynomial of $\xi,\kappa,\sigma,\sigma^{-1},\rho_1,\dots,\rho_5$ with coefficients bounded above by some absolute constants independent of $\kappa,c,d$. Since all terms in $\xi,\kappa,\sigma,\sigma^{-1},\rho_1,\dots,\rho_5$ are bounded above by some absolute constants, then so is $\frac{\partial^5 (d'\kappa)}{\partial \kappa^5}(x)$ for all $x\in[0,\kappa]$.
Thus there exists some constant $K_d$ independent of $c,d,\kappa$ such that $\abs{R_d(\kappa)}\leq K_d.$
%\frac{10080 \kappa^3}{\alpha^7}+\frac{262080 \kappa^7}{\alpha^{11}}+\frac{1774080 \kappa^{11}}{\alpha^{15}}+\frac{3548160 \kappa^{15}}{\alpha^{19}}+\alpha  \rbr{-\frac{3360 \kappa^{15} \xi}{\sigma^9}-\frac{7200 \kappa^{11} \xi}{\sigma^7}-\frac{4680 \kappa^7 \xi}{\sigma^5}-\frac{840 \kappa^3 \xi}{\sigma^3}}+d \kappa  \rbr{-\frac{3360 \kappa^{15} \xi}{\sigma^9}-\frac{7200 \kappa^{11} \xi}{\sigma^7}-\frac{4680 \kappa^7 \xi}{\sigma^5}-\frac{840 \kappa^3 \xi}{\sigma^3}}+5 d \rbr{-\frac{240 \kappa^{12} \xi}{\sigma^7}-\frac{432 \kappa^8 \xi}{\sigma^5}-\frac{204 \kappa^4 \xi}{\sigma^3}-\frac{12 \xi}{\sigma}}-\frac{20 \kappa^3 \rbr{-\frac{240 \kappa^{12} \xi}{\sigma^7}-\frac{432\kappa^8 \xi}{\sigma^5}-\frac{204 \kappa^4 \xi}{\sigma^3}-\frac{12 \xi}{\sigma}}}{\alpha^3}+10 \rbr{-\frac{24 \kappa^9 \xi}{\sigma^5}-\frac{36 \kappa^5 \xi}{\sigma^3}-\frac{12 \kappa  \xi}{\sigma}} \rho_2+10 \rbr{-\frac{4 \kappa^6 \xi}{\sigma^3}-\frac{6 \kappa^2 \xi}{\sigma}} \rho_3-\frac{10 \kappa^3 \xi  \rho_4}{\sigma}+\sigma  \rho_5

==> Sec4_EoS_Condition/general_scalar_nets.tex <==
\begin{minipageparskip}{0.6\textwidth}

Now we look into an interesting example with different behaviors around different EoS minima.
We consider a 3-layer scalar network with objective $\min_{x,y,z\in R}\frac12(1 - xyz)^2$ and initialization with $z=y$. The equality of the last two entries will be preserved through training so the dynamics is two dimensional in terms of $x$ and $y$. In the positive quadrant, the global minima is $\sqrt{x}y=1$ and there are two EoS minima.
In \cref{fig:MT-3Num-EoS-region}, we plot the converging sharpness from different initializations in comparison with \cref{fig:MT-prelim-eos-exp-region} and \cref{fig:MT-sec4-2num-noEoS-exp-region}.

Around the EoS minimum that the single entry $x$ is small and the duplicated entries $y$ are large (upper left of \cref{fig:MT-3Num-EoS-region}), the behavior is similar to the 2 scalar case (\cref{fig:MT-sec4-2num-noEoS-exp-region}) with no sharpness concentration. Around the EoS minima with large single entry and small duplicating entries (lower right of \cref{fig:MT-3Num-EoS-region}), we have a region of initialization (the red shaded area) with sharpness concentration similar to the 4 scalar case (\cref{fig:MT-prelim-eos-exp-region}).

\end{minipageparskip}\hfill
\begin{minipageparskip}{0.34\textwidth}
\begin{figure}[H]
\begin{center}
\vskip -14pt
\includegraphics[width=0.85\textwidth]{Figures/general_scalar_eos/eos_boundary_3num_fig.pdf}
\end{center}
\vskip -5pt
\caption{Converging sharpness of $(x,y,y)$ parameterized initializations ($\eta=0.2$).}
\label{fig:MT-3Num-EoS-region}
\end{figure}
\end{minipageparskip} 

A heuristic explanation to this difference lies in the difference in the degree of the small entries. Around the EoS minima that the single entry is small, the local two-step approximation is similar to \cref{eqn:MT-2Num-2step-dynamics} and gives us elliptical two-step trajectories. Around the minima with small duplicating entries, the two-step approximation would contain the cubic term as in \cref{eqn:MT-ab-dynamics-approx}, which gives us both sharpness concentration and adaptivity. We note that empirically similar phenomenon is also true for more general scalar networks without symmetric initializations. See %The relevant empirical results and discussions are deferred to 
\cref{sec:APDX-exp-general-scalar-net}.

% When there are multiple ``large'' entries or more than 2 ``smallest'' entries, this observation still holds \xiang{it's a bit confusing}.

% \rnote{Please rewrite this to focus on the degree-3 setting and defer general case to appendix. We don't have enough space here to discuss this in detail. Just show the picture and talk about how it's like degree-2 on one side and degree-3 on another side.}
% Now we briefly discuss some empirical observations on general $n$-layer scalar networks parameterized by $x_1, \dots, x_n\in \R$ with objective $\cL(x_1,\dots,x_n)\triangleq \tfrac12(1-\Pi_{i=1}^nx_i).$
% % \begin{equation}
% %     \cL(x_1,\dots,x_n)\triangleq \tfrac12(1-\Pi_{i=1}^nx_i)
% % \end{equation}

% \textbf{(a). When EoS happens, multiple small entries are equal}.\\
% We use a 3 scalar example with symmetric initialization $(x, y, y)$ \xiang{why is this symmetric?}\znote{partial symmetry?} to demonstrate this observation. As shown in \cref{fig:MT-3Num-EoS-region}, 

% \textbf{(b). Different small entries quickly converge to be equal.}\\
% When the initialization contains multiple small unequal entries and at least one large entry,  the small entries quickly converge to be equal and reduce to case (a). We will discuss the characterization of ``small'' and ``large'' entries in more detail in \cref{sec:APDX-exp-general-scalar-net-smallvslarge}.
% \znote{Might want to conclude sec4 by writing some "condition"}
